Determination of the angular momentum distribution of supernovae from gravitational wave observations

Significant progress has been made in the development of an international network of gravitational wave detectors, such as TAMA300, LIGO, VIRGO, and GEO600. For these detectors, one of the most promising sources of gravitational waves are core collapse supernovae especially in our Galaxy. Recent simulations of core collapse supernovae, rigorously carried out by various groups, show that the features of the waveforms are determined by the rotational profiles of the core, such as the rotation rate and the degree of the differential rotation prior to core-collapse. Specifically, it has been predicted that the sign of the second largest peak in the gravitational wave strain signal is negative if the core rotates cylindrically with strong differential rotation. The sign of the second peak could be a nice indicator that provides us with information about the angular momentum distribution of the core, unseen without gravitational wave signals. Here we present a data analysis procedure aiming at the detection of the second peak using a coherent network analysis and estimate the detection efficiency when a supernova is at the sky location of the Galactic center. The simulations showed we were able to determine the sign of the second peak under an idealized condition of a network of gravitational wave detectors if a supernova occurs at the Galactic center.

==> Makefile <==
LATEX=latex
DVIPS=dvips
BIBTEX=bibtex
DVIPDF=dvipdfmx
TEXFILE=secondpeak

build:
	${LATEX} ${TEXFILE}.tex
	${BIBTEX} ${TEXFILE}
	${LATEX} ${TEXFILE}.tex
	${LATEX} ${TEXFILE}.tex
	${DVIPDF} ${TEXFILE}.dvi
view:
#	open -a Adobe\ Reader ${TEXFILE}.pdf &
	open -a preview ${TEXFILE}.pdf &
print:
	lpr -Plp ${TEXFILE}.ps
#miniprint:
#	psnup -2 ${TEXFILE}.ps | psprint -flip -
pdf:
	ps2pdf ${TEXFILE}.ps
edit	:
	mate $(TEXFILE).tex
clean:
	rm -f ${TEXFILE}.log ${TEXFILE}.aux ${TEXFILE}.log ${TEXFILE}.dvi ${TEXFILE}.bbl ${TEXFILE}.blg ${TEXFILE}.toc *~

